Towards using Few-Shot Prompt Learning for Automating Model Completion

We propose a simple yet a novel approach to improve completion in domain modeling activities. Our approach exploits the power of large language models by using few-shot prompt learning without the need to train or fine-tune those models with large datasets that are scarce in this field. We implemented our approach and tested it on the completion of static and dynamic domain diagrams. Our initial evaluation shows that such an approach is effective and can be integrated in different ways during the modeling activities.

==> ICSE NIER'23 - Model autocompletion/sections/Conclusions.tex <==
We proposed a novel approach based on few-shot prompt learning to enable large language models to solve completion tasks in modeling activities. We reformulate model completion as a semantic mapping problem that consists, firstly, in transforming modeling formalism elements into meaningful patterns of sequences of tokens to create prompts with learning shots. Then, we exploit the ability of LLMs to complete partial sequences following the specified patterns to recover elements that can be used for the completion. Those elements are transformed into constructs conforming to the modeling language syntax and suggested to the designers.  
Although many research contributions were proposed to solve model completion problems, we do believe that none of them can be effectively used in a real setting, because of the resources needed, i.e., large training datasets, and the limited performance they offer. We do believe, however, that our approach can be effective when modeling both static and dynamic diagrams for two main reasons. Firstly, it does not require to pre-train or fine tune language models on specific tasks or domain. Secondly, the used LLMs are trained on a huge volume of data, which makes it generalizable to many domains and different concept natures and relationships. 

Although our approach shows promising results, it is still a first attempt and there is room for improvement. Indeed, when defining a prompt, the elements of the already-defined partial diagrams have a great influence on the accuracy of the suggested token. A calibration study is still necessary to determine the boundaries of the provided existing context to have the best suggestions. For example, when we added systematically the package name in the pattern, the results improved considerably, but we cannot determine whether this observation is valid only on the used benchmark.
Another consideration that has to be studied is the use of non-natural language elements such as symbols and digits. In our experiments, their existance generated poor results as these elements are rarely present in the data used for training LLM. We believe that a more sophisticated mapping of those elements would considerably improve the results.
%Another aspect worth investigating is the number of shots necessary to generate optimal results.
Using LLMs proves to be efficient in modeling formalism that rely heavily on natural language identifiers. However, other modeling languages such as Petri nets are definitely difficult to handle as they involve modeling elements that cannot be captured by LLMs. 

In summary, the proposed approach, although simple to implement, is powerful and showed promising results. Those results are possibly even better if we consider the fact that the boundaries of a domain are broader than the diagrams we considered as ground truth in our experiments. In fact, some of the suggested elements, although absent in the considered diagrams may be relevant for the considered domain. To asses such a claim, we plan to conduct a user study to better assess the correctness of the suggestions, but also the usefulness of the completion for the domain modelers.

==> ICSE NIER'23 - Model autocompletion/sections/intro.tex <==
%Intro and related work... \cite{RoccoSRN21}


%Prompt learning to move from the semantics of Natural Language (NL) to the semantics of a formalism. In our case, we illustrate it with class diagrams and activity diagrams...

Recent developments in deep learning-based language models (LMs) open a world of possibilities to automate and assist software specialists in software development and maintenance tasks.
At the implementation level, large code bases allow us to leverage these language models by pre-training them to have good code representations and by fine-tuning them on software engineering specific tasks.

These opportunities are, however, limited when dealing with early software development phases such as analysis and design. Datasets are scarce, and when available, they are not large enough to pre-train or fine-tune deep-learning models.
For software modeling activities, several contributions were proposed to circumvent the lack of large datasets. The goal of these research contributions is to recommend domain concepts, their features, and relationships during modeling activities\footnote{Note that ``deep-learning/language model'' and ``software model'' do not refer to the same type of model. To avoid confusion, in this work, each time we refer to a deep-learning or language model (LM), we always refer to it as such, and never as ``model'' alone.}.

Di Rocco et al.~\cite{RoccoSRN21} proposed an approach based on graph kernels that only need a small-size dataset for training. Although the results were promising, the quality of the recommended elements remains too low to be used in real settings.
Similarly, Weyssow et al.~\cite{WeyssowSS22}, used such model/metamodel datasets to train an LSTM neural network. Here again, the authors obtained limited results, especially when applied to the iterative construction of a metamodel.
From another perspective, Capuano et al.~\cite{Capuano22}, exploited the available large code bases to reverse-engineering a set of models to train a RoBERTa language model. The results are acceptable, but the  reverse-engineered models on which the authors had to rely for training led to suggestions that reflect implementation aspects rather than the modeled domains.
%Always with the perspective of exploiting other source of data,
With the goal of exploiting knowledge captured in general and specific natural-language documents, Burgueño et al.~\cite{Burgueno21} used these documents to train language models to suggest model completions. We believe that exploiting natural-language sources is a good idea to overcome the scarcity of the data to exploit deep-learning to assist in modeling activities. However, this work requires to train a language model from scratch for each specific domain, which remains a challenging problem in many scenarios.

In this paper, we propose the novel idea of exploiting powerful left-to-right large language models (LLMs). %(Brown et al. NeurIPS 2020).
To this end, we use few-shot prompt learning, which allows us to exploit these LLMs without having to train or fine-tune them on a specific domain or task, and which has proven its efficiency to various natural language processing tasks~\cite{Liu22}. %(Liu et al. ACM Comp. Survey 2022).  This technique consists in giving very few examples (few shots) on the kind of information we are looking for and then give a specific text to complete (which we will call \emph{query}). 
For example, %In the following, we present a simple example where we explain these concepts. 
if the goal is to use a LLM to generate the name of the capital of a given country, we need to prepare a prompt where we first provide the LM a description on how to reply to our queries, then we add relevant labeled samples such as two countries and their corresponding capitals (two shots). Finally, we give the country for which we want the LM to provide its capital, i.e., autocomplete. Figure \ref{fig:conceptsQuery} gives an overview on how to use LLM with prompt learning, with the example of countries and capitals. Note that apart from being an autocomplete engine, these language models are also pattern matching and pattern generation engines. This is why we need to provide not only information about the task to perform but also the pattern that we want them to replicate.
%In our example, each prediction unit is a token or span and not an entire text, as a result it is recommended to put the max tokens parameters to a low value.
%The generated text will try to fit the pattern in accordance with how the prompt  is written.
As our example shows, the generated text could include further information. For instance, \texttt{Japan => Tokyo} has also been generated, which is not of our interest. To deal with this behaviour, properly transforming queries into prompts and results into modeling elements is an essential part of the approach.


\begin{figure}[h]
\begin{center} 
\includegraphics[width=0.45\textwidth]{figures/ToyExample2.png}
\caption{Explanatory example}
\label{fig:conceptsQuery}
\vspace{-4mm}
\end{center}
\end{figure}

We specifically take advantage of GPT-3, which is one of the most powerful LM (which contains 175 billion parameters~\cite{BrownMRSKDNSSAA20}), to represent most of the existing general concepts to support software specialists when modeling. To adapt the semantics of the general concepts represented in GPT-3 to the semantics of modeling formalisms, we use two semantic mappings: one that takes the model under construction (i.e., the input to our system) and builds the prompt, and another one that obtains model auto-completion suggestions from the text produced by the language model. These semantic mappings rely heavily on the targeted modeling formalisms.

In this new-ideas paper, we illustrate our approach with two examples coming from two categories of modeling languages: static models, i.e., UML class diagrams; and dynamic models, i.e., UML activity diagrams. We propose an initial implementation of this idea and a preliminary evaluation.

